Implementing the Stochastics Brane Calculus in a Generic Stochastic Abstract Machine

In this paper, we deal with the problem of implementing an abstract machine for a stochastic version of the Brane Calculus. Instead of defining an ad hoc abstract machine, we consider the generic stochastic abstract machine introduced by Lakin, Paulev\'e and Phillips. The nested structure of membranes is flattened into a set of species where the hierarchical structure is represented by means of names. In order to reduce the overhead introduced by this encoding, we modify the machine by adding a copy-on-write optimization strategy. We prove that this implementation is adequate with respect to the stochastic structural operational semantics recently given for the Brane Calculus. These techniques can be ported also to other stochastic calculi dealing with nested structures.

==> eptcsdata.tex <==
\providecommand{\firstpage}{82}
\providecommand{\publicationstatus}{Gabriel Ciobanu (Ed.): Membrane Computing and\\ 
Biologically Inspired Process Calculi (MeCBIC 2012)\\
EPTCS 100, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.100.6}{10.4204/EPTCS.100.6}}
\pdfoutput=1

